Incorporating Terminology Constraints in Automatic Post-Editing

Users of machine translation (MT) may want to ensure the use of specific lexical terminologies. While there exist techniques for incorporating terminology constraints during inference for MT, current APE approaches cannot ensure that they will appear in the final translation. In this paper, we present both autoregressive and non-autoregressive models for lexically constrained APE, demonstrating that our approach enables preservation of 95% of the terminologies and also improves translation quality on English-German benchmarks. Even when applied to lexically constrained MT output, our approach is able to improve preservation of the terminologies. However, we show that our models do not learn to copy constraints systematically and suggest a simple data augmentation technique that leads to improved performance and robustness.

==> result_ape.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{l l c c c c }
\hline
 & term\% & TER & BLEU  & time (sent/s) \\
\hline
Do-nothing & 94.00 & 24.32 & 62.88 & \\
\hline
Transformer (\textit{src} + \textit{mt} $\to$ \textit{pe}) & 95.36 & 19.74 & 70.35 & \\
Trans Term ( \textit{src} + \textit{mt} + \textit{term} $\to$ \textit{pe} ) & 98.32	& 19.16 & 70.79 & \\
Trans Term app. ( \textit{src\_app} + \textit{mt} $\to$ \textit{pe} ) & 98.54 & 19.08 & 71.33 & \\
Trans Term rep. ( \textit{src\_rep} + \textit{mt} $\to$ \textit{pe} ) & 98.94 & 19.04 & 71.11 & \\
\hline
LevT (\textit{src} $\to$ \textit{mt} : \textit{pe}) & 94.62	& 23.14 &	66.26 & \\
LevT + mt ( \textit{src} + \textit{mt} $\to$ \textit{term} : \textit{pe} ) & 98.98 & 20.47 & 69.48 & 12.48 \\
LevT Term ( \textit{src} + \textit{term} $\to$ \textit{mt} : \textit{pe} ) & 95.14 & 23.15 & 66.37 \\
LevT Term app. ( \textit{src\_app} $\to$ \textit{mt} : \textit{pe} ) & 94.97 & 23.11 & 65.98 & \\
LevT Term rep. ( \textit{src\_rep} $\to$ \textit{mt} : \textit{pe} ) & 95.28 & 22.93 & 66.27 & 37.17\\

\end{tabular}
\end{center}
\caption{\label{result_ape} Result }
\end{table}

==> result_distillation.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c c c c c}
\hline
Pretrain & Finetune & term\% & TER & BLEU \\
\hline
 - & - & 98.04 & 17.71 & 73.64 \\
 - & ft. &  97.72 & 17.91 & 73.26 \\
 - & app. &  97.72 & 17.87 & 73.31 \\
 pre. & - & 99.09 & 17.17 & 74.40 \\
 pre. & ft. &  \textbf{99.54}  & 17.09 & 74.29\\
 pre. & app. &  \textbf{99.54} & 17.07 & 74.32 \\
 ft. & - &  96.81 & 17.06 & 74.48 \\
 ft. & ft. & 96.13 & 17.04 & 74.48 \\
 ft. & app. &  96.13 & \textbf{17.02} & \textbf{74.52} \\
 app. & - &  98.41 & 17.11 & 74.40 \\
 app. & app. &  98.86 & 17.24 & 74.04 \\

\end{tabular}
\end{center}
\caption{\label{result_distillation} Experiments with distillation. We show the distillation teacher for pretraining and finetuning. The teachers include pretrained baseline model (pre.), finetuned baseline model (ft.), and the append method (app.). }
\end{table}

==> result_nmt_regular.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{l c c c c }
\toprule
 & Term\% & TER & BLEU  &  \\
\midrule
Do-nothing & 90.22 & 16.84 & 74.73 \\
Unbabel\_BERT & 89.98  & \textbf{16.06} & \textbf{75.96}  \\
\midrule
MST & 90.66 & 16.46 & 75.61 \\
MST Append  & 90.89 & 16.57 & 75.21 \\
MST Replace & 89.98 & 16.42 & 75.65 \\
\midrule
MS LevT & 89.98 & 17.17 & 74.46 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{result_nmt_regular} Results for NMT 2019. The constrained systems do not receive any terms as input. }
\end{table}

==> result_pbmt_2017.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{l c c c c }
\hline
 & term\% & TER & BLEU   \\
\hline
Do-nothing & 88.83 & 24.48 & 62.49 \\
\hline
MST  & 90.83 & 18.83 & 71.07 \\
MST Append  & 95.83 & 18.60 & 71.02 \\
MST Replace & 95.50 & 19.13 & 70.61 \\
\hline
LevT  & 89.50 & 24.45 & 65.31\\
LevT App. & 91.00 & 24.04 & 64.80 \\
LevT Rep.  & 91.00 & 23.76 & 65.31 \\
MS LevT & 98.17 & 20.53 & 68.66\\

\end{tabular}
\end{center}
\caption{\label{result_pbmt_2017} Results for PBMT 2017.  }
\end{table}

==> result_pbmt_regular.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{l c c c c }
\toprule
 & Term\% & TER & BLEU   \\
\midrule
Do-nothing & 88.48 & 24.25 & 62.99 \\
MS\_UEdin\ & 88.70 & \textbf{18.01} & \textbf{72.52} \\
\midrule
MST & 90.11 & 19.34 & 70.44 \\
MST Append & \textbf{91.50} & \textbf{18.77} & \textbf{70.85} \\
MST Replace & 90.90 & 19.25 & 70.53 \\
\midrule
LevT  & 90.76 & 24.21 & 63.47 \\
LevT App & 89.17 & 24.10 & 64.72 \\
LevT Rep  & 89.17 & 23.76 & 65.27 \\
MS LevT & 89.83 & 20.59 & 68.59 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{result_pbmt_regular} Results for PBMT 2018. The constrained systems do not receive any terms as input.  }
\end{table}
